AdaptiveFusion: Adaptive Multi-Modal Multi-View Fusion for 3D Human Body Reconstruction

Recent advancements in sensor technology and deep learning have led to significant progress in 3D human body reconstruction. However, most existing approaches rely on data from a specific sensor, which can be unreliable due to the inherent limitations of individual sensing modalities. Additionally, existing multi-modal fusion methods generally require customized designs based on the specific sensor combinations or setups, which limits the flexibility and generality of these methods. Furthermore, conventional point-image projection-based and Transformer-based fusion networks are susceptible to the influence of noisy modalities and sensor poses. To address these limitations and achieve robust 3D human body reconstruction in various conditions, we propose AdaptiveFusion, a generic adaptive multi-modal multi-view fusion framework that can effectively incorporate arbitrary combinations of uncalibrated sensor inputs. By treating different modalities from various viewpoints as equal tokens, and our handcrafted modality sampling module by leveraging the inherent flexibility of Transformer models, AdaptiveFusion is able to cope with arbitrary numbers of inputs and accommodate noisy modalities with only a single training network. Extensive experiments on large-scale human datasets demonstrate the effectiveness of AdaptiveFusion in achieving high-quality 3D human body reconstruction in various environments. In addition, our method achieves superior accuracy compared to state-of-the-art fusion methods.

==> sections/biography.tex <==
% \vspace{-10 mm}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/anjunchen.jpg}}]{Anjun Chen} received the B.S. degree from the College of Communication Engineering of Jilin University, Changchun, China, in 2019. He is currently pursuing the Ph.D. degree with the College of Control Science and Engineering of Zhejiang University, Hangzhou, China. His research interests lie in 3D human body reconstruction and multi-modal fusion.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/xiangyuwang.jpg}}]{Xiangyu Wang} received the B.S. degree in control science and engineering from Zhejiang University, Hangzhou China, in 2021. He is currently pursuing the M.S. degree in control science with the College of Control Science and Engineering at Zhejiang University, Hangzhou, China. His research interests lie in 3D reconstruction and neural rendering.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/zhixu.jpg}}] {Zhi Xu} receives her B.S. degree from Zhejiang University in 2024, and then goes to University of California San Diego to study for a Master of Science in Computer Science. Her research interests are in vision-language models and autonomous driving scene recognition.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/kunshi.jpg}}] {Kun Shi} received the B.S. degree in electrical engineering and automation from the Nanjing University of Science and Technology, Nanjing, China, in 2018. He is currently working toward the Ph.D. degree in control science and engineering with the College of Control Science and Engineering, Zhejiang University, Hangzhou, China.
His research interests include multi-target tracking, state estimation, information fusion, autonomous driving, and wireless sensor networks.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/yanqin.png}}] {Yan Qin} received the B.S. degree in electronic information engineering from Information Engineering University, Zhengzhou, China, in 2011, the M.S. degree in control theory and control engineering from Northeastern University, Shenyang, China, in 2013, and the Ph.D. degree in control science and engineering from Zhejiang University, Hangzhou, China, in 2018. From 2019 to 2022, he was a Postdoctoral Research Fellow with the Singapore University of Technology and Design and the Nanyang Technological University, respectively. He is currently a Professor with the School of Automation, Chongqing University, Chongqing, China. His research interests include vehicle trajectory prediction in the V2X network, data-driven process monitoring, soft sensor modeling, and remaining useful life estimation for industrial processes and essential assets.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/yuchihuo.jpg}}]{Yuchi Huo} is a ”Hundred Talent Program” researcher in State Key Lab of CAD\&CG, Zhejiang University. His research interests are in neural rendering, 3D computational vision, and optical neural networks, which are aiming for the realization of next-generation neural rendering pipeline and physical-neural computation.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/cjm.jpg}}]{Jiming Chen} is a Changjiang Scholars Professor with College of control science and engineering, Zhejiang University. He is vice Dean of Facutly of Information Technology,  deputy director of the State Key laboratory of Industrial Control Technology, Director of Industrial Process Control. He was a visiting researcher at University of Waterloo from 2008 to 2010. Currently, He serves/served associate editors for ACM TECS, IEEE TPDS, IEEE Network, IEEE TCNS, IEEE TII, etc. He has been appointed as a distinguished lecturer of IEEE Vehicular Technology Society 2015, and selected in National Program for Special Support of Top-Notch Young Professionals, and also funded Excellent Youth Foundation of NSFC. He also was the recipients of IEEE INFOCOME 2014 Best Demo Award, IEEE ICCC 2014 best paper award, IEEE PIMRC 2012 best paper award, and JSPS Visiting Fellowship 2011. He also received the IEEE Comsoc Asia-pacific Outstanding Young Researcher Award 2011. He is a Distinguished Lecturer of IEEE Vehicular Technology Society (2015-2018), and a Felllow of IEEE. His research interests include networked control, sensor networks, cyber security, IoT.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/qiye.jpg}}]{Qi Ye} is a Tenure-Track Professor under the Hundred Talents Program at Zhejiang University. Before joining Zhejiang University in 2020, She was a research scientist of Mixed Reality \& AI Lab at Cambridge, Microsoft. Prior to joining Microsoft, she was a Ph.D. student at Imperial Computer Vision and Learning Lab of Imperial College London, under the supervision of Tae-Kyun Kim. She obtained her Master's degree from the School of Information Science and Technology of Tsinghua University in 2014 and a Bachelor's degree from the College of Information Science and Technology of Beijing Normal University in 2011. She is interested in and working on human-computer interaction, particularly vision understanding involving hands, and a more general setting where humans interact with the environment. She is passionate about 3D vision and their applications, particularly in Mixed/Augmented/Virtual Reality and automatic control.
\end{IEEEbiography}

